Should we agree to disagree about Twitter's bot problem?

Bots, simply defined as accounts controlled by automation, can be used as a weapon for online manipulation and pose a threat to the health of platforms. Researchers have studied online platforms to detect, estimate, and characterize bot accounts. Concerns about the prevalence of bots were raised following Elon Musk's bid to acquire Twitter. Twitter's recent estimate that 5\% of monetizable daily active users being bot accounts raised questions about their methodology. This estimate is based on a specific number of active users and relies on Twitter's criteria for bot accounts. In this work, we want to stress that crucial questions need to be answered in order to make a proper estimation and compare different methodologies. We argue how assumptions on bot-likely behavior, the detection approach, and the population inspected can affect the estimation of the percentage of bots on Twitter. Finally, we emphasize the responsibility of platforms to be vigilant, transparent, and unbiased in dealing with threats that may affect their users.

==> table-1.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c||c|c|c||c|c|c}
        \hline
        Sources & Tweet & Follow & Mention & Private & Suspended & Deleted \\
        \hline
        Stream API & \cmark & & \cmark & \xmark & \cmark & \cmark \\
        Network Crawl &  & \cmark & & \cmark & \xmark & \xmark\\
        Search API & \cmark & & \cmark & \xmark & \xmark & \xmark\\
        \hline
        Twitter mDAU & \cmark & & & \cmark & \xmark & \xmark\\
        Twitter DB & & & & \cmark & \cmark & \cmark \\
        \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
